A $\gamma$-ray determination of the Universe's star-formation history

The light emitted by all galaxies over the history of the Universe produces the extragalactic background light (EBL) at ultraviolet, optical, and infrared wavelengths. The EBL is a source of opacity for $\gamma$ rays via photon-photon interactions, leaving an imprint in the spectra of distant $\gamma$-ray sources. We measure this attenuation using {739} active galaxies and one gamma-ray burst detected by the {\it Fermi} Large Area Telescope. This allows us to reconstruct the evolution of the EBL and determine the star-formation history of the Universe over 90\% of cosmic time. Our star-formation history is consistent with independent measurements from galaxy surveys, peaking at redshift $z\sim2$. Upper limits of the EBL at the epoch of re-ionization suggest a turnover in the abundance of faint galaxies at $z\sim 6$.

==> Archive 2/auth_list.tex <==
\noindent
S.~Abdollahi$^{1}$, 
M.~Ackermann$^{2}$, 
M.~Ajello$^{3}\dagger$, 
W.~B.~Atwood$^{4}$, 
L.~Baldini$^{5}$, 
J.~Ballet$^{6}$, 
G.~Barbiellini$^{7,8}$, 
D.~Bastieri$^{9,10}$, 
J.~Becerra~Gonzalez$^{11,12}$, 
R.~Bellazzini$^{13}$, 
E.~Bissaldi$^{14,15}$, 
R.~D.~Blandford$^{16}$, 
E.~D.~Bloom$^{16}$, 
R.~Bonino$^{17,18}$, 
E.~Bottacini$^{16,19}$, 
S.~Buson$^{11}$,
J.~Bregeon$^{20}$, 
P.~Bruel$^{21}$, 
R.~Buehler$^{2}$, 
R.~A.~Cameron$^{16}$, 
R.~Caputo$^{22}$, 
P.~A.~Caraveo$^{23}$, 
E.~Cavazzuti$^{24}$, 
E.~Charles$^{16}$, 
S.~Chen$^{9,19}$, 
C.~C.~Cheung$^{25}$, 
G.~Chiaro$^{23}$, 
S.~Ciprini$^{26,27}$, 
J.~Cohen-Tanugi$^{20}$, 
L.~R.~Cominsky$^{28}$, 
J.~Conrad$^{29,30}$, 
D.~Costantin$^{10}$, 
S.~Cutini$^{26,27}$, 
F.~D'Ammando$^{31,32}$, 
F.~de~Palma$^{15,33}$, 
A.~Desai$^{3}\dagger$, 
S.~W.~Digel$^{16}$, 
N.~Di~Lalla$^{5}$, 
M.~Di~Mauro$^{16}$, 
L.~Di~Venere$^{14,15}$, 
A.~Dom\'inguez$^{34}\dagger$, 
C.~Favuzzi$^{14,15}$, 
S.~J.~Fegan$^{21}$, 
J.~Finke$^{25}\dagger$, 
A.~Franckowiak$^{2}$, 
Y.~Fukazawa$^{1}$, 
S.~Funk$^{35}$, 
P.~Fusco$^{14,15}$, 
G.~Gallardo~Romero$^{2,36}$, 
F.~Gargano$^{15}$, 
D.~Gasparrini$^{26,27}$, 
N.~Giglietto$^{14,15}$, 
F.~Giordano$^{14,15}$, 
M.~Giroletti$^{31}$, 
D.~Green$^{12,11}$, 
I.~A.~Grenier$^{6}$, 
L.~Guillemot$^{37,38}$, 
S.~Guiriec$^{39,11}$, 
D.~H.~Hartmann$^{3}$, 
E.~Hays$^{11}$, 
K.~Helgason$^{40,42}\dagger$, 
D.~Horan$^{21}$, 
G.~J\'ohannesson$^{41,42}$, 
D.~Kocevski$^{11}$, 
M.~Kuss$^{13}$, 
S.~Larsson$^{43,30}$, 
L.~Latronico$^{17}$, 
J.~Li$^{2}$, 
F.~Longo$^{7,8}$, 
F.~Loparco$^{14,15}$, 
B.~Lott$^{44}$, 
M.~N.~Lovellette$^{25}$, 
P.~Lubrano$^{27}$, 
G.~M.~Madejski$^{16}$, 
J.~D.~Magill$^{12}$, 
S.~Maldera$^{17}$, 
A.~Manfreda$^{5}$, 
L.~Marcotulli$^{3}$, 
M.~N.~Mazziotta$^{15}$, 
J.~E.~McEnery$^{11,12}$, 
M.~Meyer$^{16}$, 
P.~F.~Michelson$^{16}$, 
T.~Mizuno$^{45}$, 
M.~E.~Monzani$^{16}$, 
A.~Morselli$^{46}$, 
I.~V.~Moskalenko$^{16}$, 
M.~Negro$^{17,18}$, 
E.~Nuss$^{20}$, 
R.~Ojha$^{11}$, 
N.~Omodei$^{16}$, 
M.~Orienti$^{31}$, 
E.~Orlando$^{16}$, 
J.~F.~Ormes$^{47}$, 
M.~Palatiello$^{7,8}$, 
V.~S.~Paliya$^{3}\dagger$, 
D.~Paneque$^{48}$, 
J.~S.~Perkins$^{11}$, 
M.~Persic$^{7,49}$, 
M.~Pesce-Rollins$^{13}$, 
V.~Petrosian$^{16}$, 
F.~Piron$^{20}$, 
T.~A.~Porter$^{16}$, 
J.~R.~Primack$^{4}$, 
G.~Principe$^{35}$, 
S.~Rain\`o$^{14,15}$, 
R.~Rando$^{9,10}$, 
M.~Razzano$^{13,51}$, 
S.~Razzaque$^{50}$, 
A.~Reimer$^{51,16}$, 
O.~Reimer$^{51,16}$, 
P.~M.~Saz~Parkinson$^{4,52,53}$, 
C.~Sgr\`o$^{13}$, 
E.~J.~Siskind$^{54}$, 
G.~Spandre$^{13}$, 
P.~Spinelli$^{14,15}$, 
D.~J.~Suson$^{55}$, 
H.~Tajima$^{56,16}$, 
M.~Takahashi$^{48}$, 
J.~B.~Thayer$^{16}$, 
L.~Tibaldo$^{57,58}$, 
D.~F.~Torres$^{59,60}$, 
E.~Torresi$^{61}$, 
G.~Tosti$^{27,62}$, 
A.~Tramacere$^{63}$, 
E.~Troja$^{11,12}$, 
J.~Valverde$^{21}$, 
G.~Vianello$^{16}$, 
M.~Vogel$^{64}$, 
K.~Wood$^{65}$, 
G.~Zaharijas$^{66,67}$
\medskip
\begin{enumerate}
\item[1.] Department of Physical Sciences, Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8526, Japan
\item[2.] Deutsches Elektronen Synchrotron DESY, D-15738 Zeuthen, Germany
\item[3.] Department of Physics and Astronomy, Clemson University, Kinard Lab of Physics, Clemson, SC 29634-0978, USA
\item[4.] Santa Cruz Institute for Particle Physics, Department of Physics and Department of Astronomy and Astrophysics, University of California at Santa Cruz, Santa Cruz, CA 95064, USA
\item[5.] Universit\`a di Pisa and Istituto Nazionale di Fisica Nucleare, Sezione di Pisa I-56127 Pisa, Italy
\item[6.] Laboratoire Astrophysique Interactions Multi-\'echelles,  Commissariat \'a l'\'energie atomique-Institute of Research into the Fundamental Laws of the Universe/Centre national de la recherche scientifique/Universit\'e Paris Diderot, Service d'Astrophysique, Commissariat \'a l'\'energie atomique Saclay, F-91191 Gif sur Yvette, France
\item[7.] Istituto Nazionale di Fisica Nucleare, Sezione di Trieste, I-34127 Trieste, Italy
\item[8.] Dipartimento di Fisica, Universit\`a di Trieste, I-34127 Trieste, Italy
\item[9.] Istituto Nazionale di Fisica Nucleare, Sezione di Padova, I-35131 Padova, Italy
\item[10.] Dipartimento di Fisica e Astronomia ``G. Galilei'', Universit\`a di Padova, I-35131 Padova, Italy
\item[11.] National Aeronautics and Space Administration Goddard Space Flight Center, Greenbelt, MD 20771, USA
\item[12.] Department of Astronomy, University of Maryland, College Park, MD 20742, USA
\item[13.] Istituto Nazionale di Fisica Nucleare, Sezione di Pisa, I-56127 Pisa, Italy
\item[14.] Dipartimento di Fisica ``M. Merlin" dell'Universit\`a e del Politecnico di Bari, I-70126 Bari, Italy
\item[15.] Istituto Nazionale di Fisica Nucleare, Sezione di Bari, I-70126 Bari, Italy
\item[16.] W. W. Hansen Experimental Physics Laboratory, Kavli Institute for Particle Astrophysics and Cosmology, Department of Physics and SLAC National Accelerator Laboratory, Stanford University, Stanford, CA 94305, USA
\item[17.] Istituto Nazionale di Fisica Nucleare, Sezione di Torino, I-10125 Torino, Italy
\item[18.] Dipartimento di Fisica, Universit\`a degli Studi di Torino, I-10125 Torino, Italy
\item[19.] Department of Physics and Astronomy, University of Padova, Vicolo Osservatorio 3, I-35122 Padova, Italy
\item[20.] Laboratoire Univers et Particules de Montpellier, Universit\'e Montpellier, Centre national de la recherche scientifique/Institut national de physique nucl\'eaire de physique des particules, F-34095 Montpellier, France
\item[21.] Laboratoire Leprince-Ringuet, \'Ecole polytechnique, Centre national de la recherche scientifique/Institut national de physique nucl\'eaire de physique des particules, F-91128 Palaiseau, France
\item[22.] Center for Research and Exploration in Space Science and Technology (CRESST) and National Aeronautics and Space Administration Goddard Space Flight Center, Greenbelt, MD 20771, USA
\item[23.] Istituto Nazionale di Astrofisica-Istituto di Astrofisica Spaziale e Fisica Cosmica Milano, via E. Bassini 15, I-20133 Milano, Italy
\item[24.] Italian Space Agency, Via del Politecnico snc, 00133 Roma, Italy
\item[25.] Space Science Division, Naval Research Laboratory, Washington, DC 20375-5352, USA
\item[26.] Space Science Data Center - Agenzia Spaziale Italiana, Via del Politecnico, snc, I-00133, Roma, Italy
\item[27.] Istituto Nazionale di Fisica Nucleare, Sezione di Perugia, I-06123 Perugia, Italy
\item[28.] Department of Physics and Astronomy, Sonoma State University, Rohnert Park, CA 94928-3609, USA
\item[29.] Department of Physics, Stockholm University, AlbaNova, SE-106 91 Stockholm, Sweden
\item[30.] The Oskar Klein Centre for Cosmoparticle Physics, AlbaNova, SE-106 91 Stockholm, Sweden
%\item[31.] Wallenberg Academy Fellow
\item[31.] Istituto Nazionale di Astrofisica Istituto di Radioastronomia, I-40129 Bologna, Italy
\item[32.] Dipartimento di Astronomia, Universit\`a di Bologna, I-40127 Bologna, Italy
\item[33.] Universit\`a Telematica Pegaso, Piazza Trieste e Trento, 48, I-80132 Napoli, Italy
\item[34.] Grupo de Altas Energ\'ias, Universidad Complutense de Madrid, E-28040 Madrid, Spain
\item[35.] Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, Erwin-Rommel-Str. 1, 91058 Erlangen, Germany
\item[36.] Circolo Astrofili Talmassons, I-33030 Campoformido (UD), Italy
\item[37.] Laboratoire de Physique et Chimie de l'Environnement et de l'Espace -- Universit\'e d'Orl\'eans / Centre national de la recherche scientifique, F-45071 Orl\'eans Cedex 02, France
\item[38.] Station de radioastronomie de Nan\c{c}ay, Observatoire de Paris, Centre national de la recherche scientifique/Institut national des sciences de l'univers, F-18330 Nan\c{c}ay, France
\item[39.] The George Washington University, Department of Physics, 725 21st St, NW, Washington, DC 20052, USA
\item[40.] Max-Planck-Institut f\"ur Astrophysik, Postfach 1317, D-85741 Garching, Germany
\item[41.] Science Institute, University of Iceland, IS-107 Reykjavik, Iceland
\item[42.] Kungliga Tekniska h{\"o}gskolan Royal Institute of Technology and Stockholm University, Roslagstullsbacken 23, SE-106 91 Stockholm, Sweden
\item[43.] Department of Physics, Kungliga Tekniska h{\"o}gskolan Royal Institute of Technology, AlbaNova, SE-106 91 Stockholm, Sweden
\item[44.] Centre d'\'Etudes Nucl\'eaires de Bordeaux Gradignan, Institut national de physique nucl\'eaire de physique des particules/Centre national de la recherche scientifique, Universit\'e Bordeaux 1, BP120, F-33175 Gradignan Cedex, France
\item[45.] Hiroshima Astrophysical Science Center, Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8526, Japan
\item[46.] Istituto Nazionale di Fisica Nucleare, Sezione di Roma ``Tor Vergata", I-00133 Roma, Italy
\item[47.] Department of Physics and Astronomy, University of Denver, Denver, CO 80208, USA
\item[48.] Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany
\item[49.] Osservatorio Astronomico di Trieste, Istituto Nazionale di Astrofisica, I-34143 Trieste, Italy
%\item[51.] Funded by contract FIRB-2012-RBFR12PM1F from the Italian Ministry of Education, University and Research (MIUR)
\item[50.] Department of Physics, University of Johannesburg, PO Box 524, Auckland Park 2006, South Africa
\item[51.] Institut f\"ur Astro- und Teilchenphysik and Institut f\"ur Theoretische Physik, Leopold-Franzens-Universit\"at Innsbruck, A-6020 Innsbruck, Austria
\item[52.] Department of Physics, The University of Hong Kong, Pokfulam Road, Hong Kong, China
\item[53.] Laboratory for Space Research, The University of Hong Kong, Hong Kong, China
\item[54.] Nycb Real-Time Computing Inc., Lattingtown, NY 11560-1025, USA
\item[55.] Purdue University Northwest, Hammond, IN 46323, USA
\item[56.] Solar-Terrestrial Environment Laboratory, Nagoya University, Nagoya 464-8601, Japan
\item[57.] Centre national de la recherche scientifique, Institut de Recherche en Astrophysique et Plan\'etologie, F-31028 Toulouse cedex 4, France
\item[58.] Galaxies Astrophysique des Hautes \'Energies Cosmologie, Universit de Toulouse, Universit\'e Paul Sabatier-Observatoire midi-pyr\'en\'ees, Institut de Recherche en astrophysique et plan\'etologie, F-31400 Toulouse, France
\item[59.] Institute of Space Sciences (Consejo Superior de Investigaciones Científicas-Institut d'Estudis Espacials de Catalunya), Campus Universitat Aut\'onoma de Barcelona, Carrer de Magrans s/n, E-08193 Barcelona, Spain
\item[60.] Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats (ICREA), E-08010 Barcelona, Spain
\item[61.] Istituto Nazionale di Fisica Nucleare-Istituto di Astrofisica Spaziale e Fisica Cosmica Bologna, via P. Gobetti 101, I-40129 Bologna, Italy
\item[62.] Dipartimento di Fisica, Universit\`a degli Studi di Perugia, I-06123 Perugia, Italy
\item[63.] INTErnational Gamma-Ray Astrophysics Laboratory Science Data Centre, CH-1290 Versoix, Switzerland
\item[64.] California State University, Los Angeles, Department of Physics and Astronomy, Los Angeles, CA 90032, USA
\item[65.] Praxis Inc., Alexandria, VA 22303, resident at Naval Research Laboratory, Washington, DC 20375, USA
\item[66.] Istituto Nazionale di Fisica Nucleare, Sezione di Trieste, and Universit\`a di Trieste, I-34127 Trieste, Italy
\item[67.] Center for Astrophysics and Cosmology, University of Nova Gorica, Nova Gorica, Slovenia
\item[$\dagger$] majello@g.clemson.edu, helgason@hi.is,
  vpaliya@g.clemson.edu,\\
  justin.finke@nrl.navy.mil, abhishd@g.clemson.edu, alberto@gae.ucm.es
\end{enumerate}
